Early Verification of Legal Compliance via Bounded Satisfiability Checking

Legal properties involve reasoning about data values and time. Metric first-order temporal logic (MFOTL) provides a rich formalism for specifying legal properties. While MFOTL has been successfully used for verifying legal properties over operational systems via runtime monitoring, no solution exists for MFOTL-based verification in early-stage system development captured by requirements. Given a legal property and system requirements, both formalized in MFOTL, the compliance of the property can be verified on the requirements via satisfiability checking. In this paper, we propose a practical, sound, and complete (within a given bound) satisfiability checking approach for MFOTL. The approach, based on satisfiability modulo theories (SMT), employs a counterexample-guided strategy to incrementally search for a satisfying solution. We implemented our approach using the Z3 SMT solver and evaluated it on five case studies spanning the healthcare, business administration, banking and aviation domains. Our results indicate that our approach can efficiently determine whether legal properties of interest are met, or generate counterexamples that lead to compliance violations.

==> ARCHIVE <==
%\begin{landscape}
    \begin{table}[h]
                %%%%%%%%%%%%%%% Table experiment 2
        \begin{subtable}{0.45\linewidth}
        { 
            \scalebox{0.6}{
            \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
                 %\hline
                 \toprule
                 %\rowcolor{lightgray!75}
                 NASA & \multicolumn{6}{|c|}{configuration 1} & & \multicolumn{6}{|c |}{configuration 2} \\
                 \cline{2-7}\cline{9-14}
                 & \multicolumn{3}{|c|}{$\mainAlg$} & \multicolumn{3}{|c|}{nuXmv} & & \multicolumn{3}{|c |}{$\mainAlg$} &  \multicolumn{3}{|c|}{nuXmv} \\
                 \cline{2-7}\cline{9-14}
                  & \multirow{2}{*}{out.} & time &   mem. & \multirow{2}{*}{out.} & time & mem.  ~&  & \multirow{2}{*}{out.} & time &  mem. &  \multirow{2}{*}{out.} & time & mem. \\ 
                   & & (sec) & (MB) &  & (sec) & (MB)  &~& & (sec) & (MB) &  & (sec) & (MB) \\
                  \cmidrule[1.5pt]{0-6}\cmidrule[1.5pt]{9-14}
                   $na_1$ & U& 0.80  & 154  &  U &  0.88 & 82 & & U & 0.13  & 141 & U & 1.65 & 90 \\\cline{2-7}\cline{9-14}
                   $na_2$ & U& 0.16 & 141 & U &  0.47 & 70 &  & U & 0.15 & 141 & U& 1.50 & 90 \\\cline{2-7}\cline{9-14}
                   $na_3$ & U& 0.16 & 141 & U & 0.49 & 83 &  & U & 0.13 & 141 & U& 1.48 & 90 \\\cline{2-7}\cline{9-14}
                   $na_4$ & U& 0.77 & 80  & U & 0.54 & 83 &  & U & 0.15 & 66 & U & 1.43 & 91 \\\cline{2-7}\cline{9-14}
                   $na_5$ & U& 0.14 & 140 & U & 0.52 & 82 & & U & 0.15 & 141 & U& 1.43 & 90 \\\cline{2-7}\cline{9-14}
                   $na_6$ & U& 0.03 & 62  & U & 0.57 & 72  & & U & 0.03 & 62 & U & 1.40 & 90
                 \\\cline{2-7}\cline{9-14}
                 \bottomrule
            \end{tabular}
            } % end scalebox
        }
        \caption{{\scriptsize \blue{Run-time performance of our approach ($\mainAlg$) and the state-of-the-art model checker (nuXmv) on the NASA case study. The configurations considered are modifying the number of ground-separated  ($\#GSEP$) and of self-separating aircraft ($\#SSEP$) as follow, configuration 1: $\#GSEP=3$ and $\#SSEP=0$; and configuration 2: $\#GSEP=2$ and $\#SSEP=2$.}}}\label{tab:effectiveness-2}
        \end{subtable}
        
        
        %%%%%%%%%%%%%%% Table experiment 3
        \begin{subtable}{0.45\linewidth} { 
            \scalebox{0.6}{
                \begin{tabular}{|c|c|c|c|c|c|}
                    \hline
                     \multirow{2}{*}{names} & \multicolumn{4}{|c|}{case study statistics} & \multirow{2}{*}{configuration values} \\\cline{2-5}
                     & $\#reqs$ & $\#rels$ & $\#args$ & $\#props$ &  \\ \hline
                     PHIM & 18 & 22 & $[1-4]$ & 7 & $\textit{\#cus}=2$, $\textit{\#pats}=2$, $\textit{\#data}=5$
                     \\ \hline
                     CF@H & 45 & 28 & $[2-3]$ & 7 & $\textit{\#usrs}=2$, $\textit{\#data}=10$
                     \\ \hline
                     PBC & 14 & 7 & $[1-2]$ & 1 & $\textit{\#usrs}=5$, $\textit{\#data}=10$
                     \\ \hline
                     \multirow{2}{*}{BST} & \multirow{2}{*}{10} & \multirow{2}{*}{3} & \multirow{2}{*}{$[1-3]$} & \multirow{2}{*}{3} & $\textit{\#empls}=1$, $\textit{\#cus}=2$\\
                         &    &   &         &   & $\textit{\#trans}=4$, $\textit{sup}=10$
                     \\ \hline
                \end{tabular}
            }
        \caption{{\scriptsize Case study statistics. The numbers of requirements, relations, relation arguments, and properties are denoted as $\#reqs$, $\#rels$, $\#args$, and $\#props$, respectively. Initial configurations with data constraints specific to each case study: PHIM -- the number of custodians ($\#cus$), patients ($\#pats$), and  data ($\#data$); CF@H and PBC -- the number of users ($\#usrs$), and data ($\#data$); BST -- the number of employees ($\#empls$), customers ($\#cus$), transactions ($\#trans$), and maximum amount for a transaction ($\textit{sup}$).}}\label{tab:models}
        }
        \end{subtable}
        \caption{AA}
        \label{tab:eAA}
        %\vspace{-0.1in}
    \end{table}
%\end{landscape}

==> archive/rebutal-cav.tex <==
We thank the reviewers for their insightful feedback and suggestions. We will address all raised concerns in the paper.

Below, we first clarify the connection between our contributions and the legal domain. We then answer the reviewers' questions individually.

\paragraph{Legal compliance}
Our goal is to verify legal compliance. To achieve this goal, we proposed a new approach for bounded MFOTL satisfiability checking. The main connection to legal compliance is the choice of the logic, MFOTL[4]. MFOTL is an expressive logic that enables the specification of data and time constraints, and it has been used for specifying legal properties [2]. Furthermore, our evaluation involves regulatory-compliance-checking case studies, specifically, BST, PBC, PHIM, and CF@H. 
Overall, we expect our core contribution, MFOTL satisfiability checking, to have even broader applications. We nonetheless elected to ground our work in the legal domain because our motivation (for choosing MFOTL) and our use cases originate from this domain.

\paragraph{Reviewer\_A}

* Regarding the novelty of the techniques used for deciding MFTOL satisfiability: 
    Thank you for pointing out the related works that use UNSAT cores for domain expansion ([Passmore-et-al-2020, Suter-et-al-2011]); we will cite them. However, there are two major differences between these and our work. First, the domains (and the over/under-approximations) are different: the above papers use UNSAT cores to identify recursive definitions to unroll. In contrast, we use UNSAT cores to identify relational objects to include in the $FOL*$ domain. Second, the usage of UNSAT cores is different:  the authors of these references select expansion candidates via fair enumeration on the UNSAT cores, whereas we use UNSAT cores to compute the minimum solution (following [28]), where candidates are used for domain expansion. Further, we have  experimented with other domain expansion strategies with or without UNSAT cores. We observed that the strategies presented in the IBS algorithm and in Remark-1 are the most effective because they try to minimize the number of relational objects added to the domain. This is important because it prevents the size of the domain and the over/under-approximation from exploding. Due to the page limit, we report only the most effective strategies. {\bf MC:  and others?} Another benefit of our IBS expansion strategy is that it enables bounded-UNSAT detection.
    
    Overall, although the general idea of using over/under-approximation and domain expansion has been explored, our formulation of over/under-approximation and our strategy for domain expansion are novel contributions for effectively deciding MFOTL satisfiability.

* Thank you for the suggestion on the compactness discussion. The compactness property does \emph{not} hold for MFOTL and $FOL*$ in general. Identifying cases where compactness holds is an interesting future work, as it makes cube-and-conquer distributed solving possible.

\paragraph{Reviewer\_B}

* Regarding [18]: This is the correct citation. The specifications in [18] use a similar form of guard quantification.

* Regarding guarded quantification: The assumption on guarded quantification is needed for the translation to FOL* (rule 3 in Fig.5). More specifically, $FOL*$ supports quantification over relational objects, and the guard assumption ensures that the translation can map the quantified value in MFOTL to a class of relational objects in FOL*.

* Clarifying Req0: The identifier (ID) of a data item must be registered (collected) in the Data Control Center (DCC) at least 15 days prior to its first access by any user. The data collection process involves providing an ID and a value for the data. A data item can be collected unconditionally, and updated if the data ID exists.

* Correcting a typo: $\forall o:r . \phi_f = \neg \exists o: r : \neg \phi_f$

* Regarding function $f: \tau \to \phi_f$: In a satisfying solution, the relational objects of class $TP$ in the $FOL*$ domain represent the finite and non-continuous time points $\tau_1, \tau_2 \ldots$. The values of $\tau_1, \tau_2 \ldots$ are given by the variable assignment on the relational objects' time attribute, which are symbolic variables in domain $\mathbb{N}$. Note that, during the translation, we do not yet have the variable assignment for determining the concrete time values. Therefore, $f$ takes a symbolic $\tau$ in the domain $\mathbb{N}$ and creates constraints based on $\tau$.

* Regarding the internal class TP: 
Although an MFOTL formula can be defined with an unbounded interval, the constraints of the formula are applied only to the finite number of time points in an MFOTL solution, $\tau_1, \tau_2, \ldots$, whose time values are in the unbounded interval. These time points are captured by the finite number of relational objects of class $TP$. 
Given a formula $\phi$, NBS (in Section 4.3) takes a bound $vb$ and tries to ground the formula considering at most $vb$  relational objects. Therefore, a satisfying solution to $\phi$ contains at most $vb$ time points whose time values are chosen by the solver to satisfy the formula. 

* Page 10: typo. n $\rightarrow$ vb

* Regarding the correctness of IBS: We stated (Thm.1) and proved the correctness of IBS (the counterexample-guided algorithm) in Appendix B.2.

* Regarding the illustration of the full algorithm: It is illustrated with an example in Appendix B.1  (as mentioned at the end of Section 5). 

* Clarification on data constraints: 
The optional data constraint is a feature -- one can add data constraints to avoid unrealistic counterexamples. During the evaluation, we use different data constraints to create different configurations (the initial data constraints are in Table 1). For each configuration, the algorithm then checks each property with bounds on data actions.  
The last configuration for each case study (last column of Table 3) does not contain any data constraints.

* Comparison against nuXmv. To compare with nuXmv, we took the models and verification properties directly from [26]. The model does contain configurations (e.g, M4-S-far-G\_far) where some properties are violated (SAT). IBS was able to verify all the properties on these configurations and find counterexamples (in less than 5 seconds). However, we cannot reproduce the result with nuXmv on these configurations using the replication instructions provided by the authors (runtime errors occurred). We contacted the first author of [26] but did not receive an answer. Therefore, for the purpose of performance comparison, we report only the results on the two configurations where nuXmv has explicitly stated support (in their README). For these configurations, all properties are UNSAT.
% For a comparison against nuXmv on SAT instances, we will experiment on a slightly mutated system configurations and report their results.\nf{NF: Discussion.}

\paragraph{Reviewer\_C}

*Regarding Definition 3: 
Given an MFOTL formula $\phi$, a trace $\sigma = (\bar{D}, \bar{\tau}, v)$ is a solution to a formula. The assignment $v$ assigns values to the variables in $\phi$ such that $(\bar{D}, \bar{\tau}, v, 0) \models \phi$ following the MFOTL semantics in Fig.~3. 

* Regarding overloading the symbol $v$: Instead of using $v$, we will use $x$ to represent variables in $V$.

* Regarding $D_{AU}$: it is a typo, $D_{AU}$ should be $D$.

* Regarding the question on the data constraints: 
In the IBS algorithm,  data constraints are optional constraints on the value of data based on the datatype. The constraints can be a range or a small data set. In our experiments, the NASA case study uses a data set for specifying the possible system control modes and uses a data range to restrict the possible measure from the aircraft (e.g., aircraft's trajectory). In the other cases studies, data constraints are data ranges (e.g., a patient's account balance should be non-negative).

* Regarding the effects of data constraints: 
For all the benchmarks, the data constraints ensure that the counterexamples contain realistic values (e.g., a valid year of birth). The data constraints are not directly related to the $FOL*$ domain. Nevertheless, the constraints can potentially restrict the options available for adding relational objects to the domain. 

==> rebutal-cav.tex <==
We thank the reviewers for their insightful feedback and suggestions. We first address the main questions regarding the paper's *scope*, *technical novelty*, and *evaluation*. We then provide further clarification about *data constraints*. Finally, we answer individual reviewer's technical questions. 

\subsection{Scope: Legal Compliance}
%====================
Reviewers A and B (RA and RB) pointed out that our work has a border range of applications, and thus wonder how our work is connected to the legal domain. We will clarify the connection below and in the paper. 
 
Our goal is to verify legal compliance. To achieve it, we propose a new approach for bounded MFOTL satisfiability checking. The main connection to legal compliance is the choice of the logic, MFOTL[4]. MFOTL is an expressive logic that enables the specification of data and time constraints, and it has been used for specifying legal properties[2]. Furthermore, our evaluation involves regulatory-compliance-checking case studies, specifically, BST, PBC, PHIM, and CF@H. 
\hl{Overall, we expect our core contribution, MFOTL satisfiability checking,  to extend to broader applications. We nonetheless chose to ground our work in the legal domain because our motivation for choosing MFOTL and our use cases originate from it.}

\subsection{Novelty: Over/Under-approximation and Core-guided Domain Expansion}
%==========================================================
RA pointed out  related work on using UNSAT-core for domain expansions (\hl{[Passmore-et-al-2020,Suter-et-al-2011]}). Thank you, and will \hl{cite it}. \hl{However, these papers do not affect our technical novelty because of two major differences: First, the domains (and the over/under-approximations) are different: the above papers use UNSAT cores to identify recursive definitions to unroll. In contrast, we use UNSAT cores to identify relational objects to include in the FOL* domain. 
Second, the usage of UNSAT cores is different:  the authors of these references select expansion candidates via fair enumeration on the UNSAT cores, whereas we use UNSAT cores to compute the minimum solution (following~[28]), where we extract relational objects as candidates for domain expansion.} 

These differences, the formulation of over and under-approximation and the strategy for the domain expansion, are important for effectively deciding MFOTL satisfibility. We have experimented with other domain expansion strategies with or without UNSAT cores. We observed  that the strategies presented in the IBS algorithm and in Remark-1 are the most effective because they try to minimize the number of relational objects added to the domain. This is important because that prevents the size of the domain and the over/under-approximation from exploding. Moreover, the IBS expansion enables bounded-UNSAT detection. 

Overall, although the high-level idea of using over/under-approximation and domain expansion has been explored, our formulation of over/under-approximation and our strategy for domain expansion are novel contributions for effectively deciding MFOTL satisfiability. We will \hl{highlight the difference in the paper}.

\subsection{Evaluation: Comparison against nuXmv}
%================================
RB wonders \st{why the benchmark instances used for the comparison against nuXmv are all UNSAT}. We clarify the reason here (and will do the same in the paper). To compare with nuXmv, we took the models and verification properties directly from [26]. Some of the models do contain configurations (e.g., M4-S-far-G\_far) where some properties are violated (and are thus SAT). IBS was able to verify all the properties on these configurations and find counterexamples, in under 5 seconds for each property. However, we were unable to reproduce this result with nuXmv on these configurations using the replication instructions provided by the authors (runtime errors occurred). We contacted the first author of [26] but did not receive an answer. Therefore, \st{for the purpose of performance comparison, we reported only on the results of the two configurations where nuXmv had explicitly stated support}. For these configurations, all properties happened to be UNSAT. Since the absence of the performance data for SAT instances raised a concern, we will extend Table~2 to report the IBS's result on all configurations.

\subsection{Confusion on Data Constraints}
%=========================
We clarify concerns expressed by RA and Reviewer C (RC) here and will do the same in the paper. 

\hl{Data constraints are *optional* constraints on the value of data based on the datatype. The constraints can be a range or a small data set. The purpose of adding data constraints is to avoid unrealistic counterexamples. For example, the NASA case study uses a data set for specifying the possible system control modes and uses data ranges to restrict the possible measures from the aircraft (e.g., aircraft's trajectory). In the other case studies, data constraints are data ranges (e.g., a patient's account balance should be non-negative).} 

During the evaluation, we use different data constraints to create different configurations (the initial data constraints are shown in Table~1). For each configuration, the algorithm IBS  checks each property with bounds on data actions.  The last configuration for each case study (last column of Table~3) does not contain any data constraints. 

\hl{Data constraints are not necessary for IBS, and to answer RC's question, they do not directly affect the FOL* domain. Nevertheless, the constraints can affect the satisfiability result by restricting the options available for adding relational objects to the domain.}

\subsection{Additional Answers}
%================
We now answer the rest of the questions asked by the reviewers.  In the paper, we will make sure to add these clarifications and fix all typos.

\subsection{Reviewer-A}
%-----------------
Compactness discussion: The compactness property does *not* apply for MFOTL and $FOL*$ in general. Some $FOl*$ instances are UNSAT in every finite domain (of relational objects), but are satisfibility in an infinite domain (and the solution has an infinite volume). On these instances, IBS would return bounded-UNSAT.    
Identifying cases where compactness does (and does not) hold is an interesting future work.

\subsection{Reviewer-C}
%-----------------
* Regarding Definition~3:  \hl{\textbf{NICK: add the clarification below to preliminary}}
\hl{Given an MFOTL formula $\phi$, a trace $\sigma = (\bar{D}, \bar{\tau}, v)$ is a solution to  it.  The assignment $v$ assigns values to the variables in $\phi$ such that $(\bar{D}, \bar{\tau}, v, 0) \models \phi$ following the MFOTL semantics in Fig.~3}. We will \hl{clarify this in the paper}.

* And, \hl{instead of overloading the symbol $v$, we will use  $x$ to represent variables in $V$.}

* Regarding \hl{$D_{AU}$: this is a typo; $D_{AU}$ should be $D$}.
 
\subsection{Reviewer-B}
%-----------------
* Regarding~[18]: This is the correct citation. The specifications in [18] use a similar form of guard quantification. 

* \hl{Regarding guarded quantification: This assumption is needed for the translation to FOL* (rule 3 in Fig.~5). More specifically, $FOL*$ supports quantification over relational objects, and the guard assumption ensures that the translation can map the quantified value in MFOTL to a class of relational objects in FOL*.} We will \hl{clarify this} in the paper.

* Clarifying Req0: The identifier (ID) of a data item must be registered (collected) in the Data Control Center (DCC) at least 15 days prior to its first access by any user. The data collection process involves providing an ID and a value for the data. A data item can be collected unconditionally and updated if the data ID exists.

* \st{Typo Correction: $\forall o:r . \phi_f = \neg \exists o: r : \neg \phi_f$.} 

* Regarding function $f: \tau \to \phi_f$: In a satisfying solution, the relational objects of class $TP$ in the $FOL*$ domain represent the finite and non-continuous time points $\tau_1, \tau_2 \ldots$. The values of $\tau_1, \tau_2 \ldots$ are given by the variable assignment on the relational objects' time attribute, which are symbolic variables in domain $\mathbb{N}$. Note that, during the translation, we do not yet have the variable assignment for determining the concrete time values. Therefore, $f$ takes a symbolic $\tau$ in the domain $\mathbb{N}$ and creates constraints based on $\tau$. We will clarify this in the paper.

* Regarding the internal class $TP$: 
Although an MFOTL formula can be defined with an unbounded interval, the constraints of the formula are applied only to the finite number of time points in an MFOTL solution, $\tau_1, \tau_2, \ldots$, whose time values are in the unbounded interval. These time points are captured by the finite number of relational objects of class $TP$. 
Given a formula $\phi$, NBS (in Section 4.3) takes a bound $vb$ and tries to ground the formula considering at most $vb$  relational objects. Therefore, a satisfying solution to $\phi$ contains at most $vb$ time points whose time values are chosen by the solver to satisfy the formula. We will clarify this in the paper.

* Page 10: typo. n $\rightarrow$ vb

* Regarding the correctness of IBS: We stated (Thm.~1) and proved the correctness of IBS (the counterexample-guided algorithm) in Appendix B.2.

* Regarding the illustration of the full algorithm: It is illustrated with an example in Appendix B.1  (as mentioned at the end of Section 5).

==> smallStatTable.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c}
    \scalebox{0.6}{
        \begin{tabular}{|c|c|c|c|c|c||c|c|c|c|c|c|}
            \toprule
             \multirow{2}{*}{names} & \multicolumn{4}{|c|}{case study statistics} & \multirow{2}{*}{configuration} & \multirow{2}{*}{names} & \multicolumn{4}{|c|}{case study statistics} & \multirow{2}{*}{configuration} \\\cline{2-5}\cline{8-11}
             & $\#reqs$ & $\#rels$ & $\#args$ & $\#props$ & & & $\#reqs$ & $\#rels$ & $\#args$ & $\#props$ &  \\ \toprule
             \multirow{2}{*}{PHIM} & \multirow{2}{*}{18} & \multirow{2}{*}{22} & \multirow{2}{*}{$[1-4]$} & \multirow{2}{*}{6} & $\textit{\#c}=2$, $\textit{\#p}=2$ &\multirow{4}{*}{NASA} & \multirow{4}{*}{194} & \multirow{4}{*}{10} & \multirow{4}{*}{$[6-79]$} & \multirow{4}{*}{6} & $\#GSEP=3$ \\
                 &    &   &         &   & $\textit{\#d}=5$
            &      &    &   &         &   & $\#SSEP=0$
             %PHIM & 18 & 22 & $[1-4]$ & 7 & $\textit{\#c}=2$, $\textit{\#p}=2$, $\textit{\#d}=5$
             \\ \cline{1-6}
             CF@H & 45 & 28 & $[2-3]$ & 7 & $\textit{\#u}=2$, $\textit{\#d}=10$
             &  &    &   &         &   & $\#GSEP=2$\\ \cline{1-6}
             \multirow{2}{*}{BST} & \multirow{2}{*}{10} & \multirow{2}{*}{3} & \multirow{2}{*}{$[1-3]$} & \multirow{2}{*}{3} & $\textit{\#e}=1$, $\textit{\#c}=2$
             &    &    &   &         &   & $\#SSEP=2$ \\\cline{7-12} %\hline
             %BST & 10 & 3 & $[1-3]$ & 3 & $\textit{\#e}=1$,$\textit{\#c}=2$,$\textit{\#t}=4$,$\textit{sup}=10$ 
             &    &   &         &   & $\textit{\#t}=4$, $\textit{sup}=10$ & PBC & 14 & 7 & $[1-2]$ & 1 & $\textit{\#u}=5$, $\textit{\#d}=10$\\
             \bottomrule
             %    &    &   &         &   & $\textit{\#t}=4$, $\textit{sup}=10$
             %\\ \hline
             % \multirow{4}{*}{NASA} & \multirow{4}{*}{194} & \multirow{4}{*}{10} & \multirow{4}{*}{$[6-79]$} & \multirow{4}{*}{6} & $\#GSEP=3$ \\
             %     &    &   &         &   & $\#SSEP=0$\\
             %     &    &   &         &   & $\#GSEP=2$\\
             %     &    &   &         &   & $\#SSEP=2$
             %\\ \hline
             %\blue{NASA} & 194 & 10 & [6-79] & 6 & $\#GSEP=3$, $\#SSEP=0$ | $\#GSEP=2, \#SSEP=2$
             %\\ \hline
        \end{tabular}
    }
    \end{tabular}
    \caption{{\footnotesize Case study statistics.}}
    \label{tab:my_label}
\end{table}

==> tabtest.tex <==
\begin{table}[t]
    \centering
            \scalebox{0.45}{
                \begin{tabular}{|c|c|c|c|c|c|}
                    \hline
                     \multirow{2}{*}{names} & \multicolumn{4}{|c|}{case study statistics} & \multirow{2}{*}{configuration values} \\\cline{2-5}
                     & $\#reqs$ & $\#rels$ & $\#args$ & $\#props$ &  \\ \hline
                     PHIM & 18 & 22 & $[1-4]$ & 7 & $\textit{\#c}=2$, $\textit{\#p}=2$, $\textit{\#d}=5$
                     \\ \hline
                     CF@H & 45 & 28 & $[2-3]$ & 7 & $\textit{\#u}=2$, $\textit{\#d}=10$
                     \\ \hline
                     PBC & 14 & 7 & $[1-2]$ & 1 & $\textit{\#u}=5$, $\textit{\#d}=10$
                     \\ \hline
                     BST & 10 & 3 & $[1-3]$ & 3 & $\textit{\#e}=1$,$\textit{\#c}=2$,$\textit{\#t}=4$,$\textit{sup}=10$ 
                     \\ \hline
                     \multirow{2}{*}{NASA} & \multirow{2}{*}{194} & \multirow{2}{*}{10} & \multirow{2}{*}{$[6-79]$} & \multirow{2}{*}{6} & $\#GSEP=3$, $\#SSEP=0$ \\
                         &    &   &         &   & $\#GSEP=2, \#SSEP=2$
                     %\\ \hline
                     %\blue{NASA} & 194 & 10 & [6-79] & 6 & $\#GSEP=3$, $\#SSEP=0$ | $\#GSEP=2, \#SSEP=2$
                     \\ \hline
                \end{tabular}\label{tab:models}
            }
    \caption{{\footnotesize Case study statistics. %\blue{Numbers of requirements, relations, relation arguments, properties: {\scriptsize$\#reqs$}, {\scriptsize$\#rels$}, {\scriptsize$\#args$}, and {\scriptsize$\#props$}.} Initial \blue{case study} configurations with data constraints: PHIM -- number of custodians ({\scriptsize$\#c$}), patients ({\scriptsize$\#p$}), data ({\scriptsize$\#d$}); CF@H and PBC -- number of users ({\scriptsize$\#u$}), data ({\scriptsize$\#d$}); BST -- number of employees ({\scriptsize$\#e$}), customers ({\scriptsize$\#c$}), transactions ({\scriptsize$\#t$}), maximum amount for a transaction ({\scriptsize$\textit{sup}$)}.
    }}
    \label{tab:stats}
\end{table}

\begin{table}[t]
    \centering
        \scalebox{0.30}{
            \begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|c|}
                 %\hline
                 \toprule
                 %\rowcolor{lightgray!75}
                 NASA & \multicolumn{6}{|c|}{configuration 1} & & \multicolumn{6}{|c |}{configuration 2} \\
                 \cline{2-7}\cline{9-14}
                 & \multicolumn{3}{|c|}{$\mainAlg$} & \multicolumn{3}{|c|}{nuXmv} & & \multicolumn{3}{|c |}{$\mainAlg$} &  \multicolumn{3}{|c|}{nuXmv} \\
                 \cline{2-7}\cline{9-14}
                  & \multirow{2}{*}{out.} & time &   mem. & \multirow{2}{*}{out.} & time & mem.  ~&  & \multirow{2}{*}{out.} & time &  mem. &  \multirow{2}{*}{out.} & time & mem. \\ 
                   & & (sec) & (MB) &  & (sec) & (MB)  &~& & (sec) & (MB) &  & (sec) & (MB) \\
                  \cmidrule[1.5pt]{0-6}\cmidrule[1.5pt]{9-14}
                   $na_1$ & U& 0.80  & 154  &  U &  0.88 & 82 & & U & 0.13  & 141 & U & 1.65 & 90 \\\cline{2-7}\cline{9-14}
                   $na_2$ & U& 0.16 & 141 & U &  0.47 & 70 &  & U & 0.15 & 141 & U& 1.50 & 90 \\\cline{2-7}\cline{9-14}
                   $na_3$ & U& 0.16 & 141 & U & 0.49 & 83 &  & U & 0.13 & 141 & U& 1.48 & 90 \\\cline{2-7}\cline{9-14}
                   $na_4$ & U& 0.77 & 80  & U & 0.54 & 83 &  & U & 0.15 & 66 & U & 1.43 & 91 \\\cline{2-7}\cline{9-14}
                   $na_5$ & U& 0.14 & 140 & U & 0.52 & 82 & & U & 0.15 & 141 & U& 1.43 & 90 \\\cline{2-7}\cline{9-14}
                   $na_6$ & U& 0.03 & 62  & U & 0.57 & 72  & & U & 0.03 & 62 & U & 1.40 & 90
                 \\\cline{2-7}\cline{9-14}
                 \bottomrule
            \end{tabular} 
            } % end scalebox
    \caption{{\footnotesize Performance comparison between  $\mainAlg$ and the nuXmv model checker on the NASA case study. 
    %The configurations considered are modifying the number of ground-separated  ({\scriptsize$\#GSEP$}) and of the self-separating aircraft ({\scriptsize$\#SSEP$}), where configuration~1 is {\scriptsize$\#GSEP=3$} and {\scriptsize$\#SSEP=0$}; and configuration~2 is {\scriptsize$\#GSEP=2$} and {\scriptsize $\#SSEP=2$}.
    }}
    \label{tab:effectiveness-2}
\end{table}

